Detecting Multi-Sensor Fusion Errors in Advanced Driver-Assistance Systems

Advanced Driver-Assistance Systems (ADAS) have been thriving and widely deployed in recent years. In general, these systems receive sensor data, compute driving decisions, and output control signals to the vehicles. To smooth out the uncertainties brought by sensor outputs, they usually leverage multi-sensor fusion (MSF) to fuse the sensor outputs and produce a more reliable understanding of the surroundings. However, MSF cannot completely eliminate the uncertainties since it lacks the knowledge about which sensor provides the most accurate data and how to optimally integrate the data provided by the sensors. As a result, critical consequences might happen unexpectedly. In this work, we observed that the popular MSF methods in an industry-grade ADAS can mislead the car control and result in serious safety hazards. We define the failures (e.g., car crashes) caused by the faulty MSF as fusion errors and develop a novel evolutionary-based domain-specific search framework, FusED, for the efficient detection of fusion errors. We further apply causality analysis to show that the found fusion errors are indeed caused by the MSF method. We evaluate our framework on two widely used MSF methods in two driving environments. Experimental results show that FusED identifies more than 150 fusion errors. Finally, we provide several suggestions to improve the MSF methods we study.

==> body/2_background.tex <==
\section{Background}
\label{sec:background}

This section provides the background for the relevant concepts and related work.
First, we categorize driving automation systems highlighting the differences between Automated Driving Systems (\ads) and Advanced Driver-{\em Assistance} Systems (\adas), where the latter is the focus of the current work.
Second, we introduce the commonly used fusion methods for driving automation systems and the ones we focus on.
Finally, we provide the background of causality analysis and the relevant notations needed to attribute the cause of an error of \adas to the fusion method used. 

%In this work, we leverage scenario-based fuzz testing on finding errors of an \adas caused by the fusion methods used. 
% In this section, we provide the background for the relevant concepts and related work.
% We start with a categorization of driving automation systems highlighting the differences between Automated Driving Systems (\ads) and \adas, where the latter is the focus of the current work.
% Next, we compare the scenario-based testing in the literature with the current work and highlight the key difference being our focus on errors caused by the fusion method used rather than general errors. 
% Following that, we introduce the commonly used fusion methods used for driving automation systems and the ones we focus on.
% Lastly, we provide the background of causality analysis as well as the relevant notations needed in order to attribute the cause of an error to the fusion method used. 

% \subsection{Terminology}
% To avoid confusions, we define the following terms adapted from \cite{scenescenariodef, scenariodefinitions}.

% \noindent
% A \textbf{Scene} is a snapshot of the current world in the simulator containing the detailed properties of all NPC vehicles and the background information.

% \noindent
% A \textbf{Logical Scenario} describes a search space of the simulation environment behavior. For example, a NPC vehicle has an initial speed $v \in [0, 10]$ m/s.

% \noindent 
% A \textbf{Specific Scenario} is a concrete instance within a \ls and it dictates the concrete behaviors of a simulation environment behavior. For example, a NPC vehicle has an initial speed $v=5$ m/s.

\subsection{{Categorization of Driving Automation Systems}}
The "Standard Road Motor Vehicle Driving Automation System Classification and Definition" %(SAE J3016(TM)) \cite{saeadlevels} 
categorizes driving automation systems into six levels (0 to 5). 
Advanced Driver-{\em Assistance} Systems (\adas) usually consists of levels 0 to 2, which only provides temporary intervention (e.g., Autonomous Emergency Braking (AEB)) or longitudianl/latitudinal control(e.g., Automated Lane Centering (ALC) and Adaptive Cruise Control (ACC)) while requiring the driver's attention all the time. 
In contrast, Automated Driving Systems (\ads) consist of Levels 3 to 5, which allow the driver to not pay attention all the time.
In the current work, we focus on \op, a level2 industry-grade \adas. However, we believe our approach can also generalize to \ads that use similar fusion methods~\cite{apollo, autoware}.



% \subsubsection{Testing for \op}
% \cite{Rubaiyat2018ExperimentalRA} studies the robustness of \op when adding noise to sensor inputs while we focus on naturally-occurred scenarios in a simulator. \cite{blackbox19} also studies \op in simulation. However, they focus on failure cases in general while we focus on finding \bugs.



% \subsubsection{Components Interaction Error Fuzzing}
% Similar to ours, \cite{interactiontest} also studies interaction error between different functionality of an \adas. However, we focus on the fusion of different perception components rather than different functionality components. Such difference leads to different design choice of the fitness function.


\subsection{\new{Fusion in Driving Automation}}

%\subsubsection{Fusion Method}
Most industry-grade driving automation systems including \adas and \ads leverage multi-sensor fusion  (\msf) to avoid potential accidents caused by the failure of a single sensor \cite{apollo, autoware, openpilot}. \msf often works with camera and radar, camera and Lidar, or the combination of camera, radar and Lidar \cite{fusionsurvey}. There are three primary types of \msf: high-level fusion (HLF), mid-level fusion (MLF), and low-level fusion (LLF). They differ in the format of the sensory data from various sensing modalities to combine.
In HLF, each sensor carries out object detection or a tracking algorithm independently. The fusion is then conducted on the high-level object attributes of the environment (e.g. the relative positions of nearby vehicles) provided by each sensor's processing module and outputs aggregate object attributes to its downstream components.
LLF fuses the sensor data at the lowest level of abstraction (raw data)\cite{llf20}.
MLF is an abstraction-level between HLF and LLF. It fuses features extracted from the sensor data, such as color information from images or location features of radar and LiDAR, and then conduct recognition and classification on them\cite{mlf15}.
Among them, HLF is particularly widely used in open-sourced commercial-grade \adas \cite{openpilot} or \ads \cite{apollo, autoware} because of its simplicity, and is our focus in the current work. 
In particular, we conduct a \carla simulator-based case study on an industry-grade \adas, \op, which uses a HLF for camera and radar. 
%We find that its fusion flow design is potentially problematic and \bugs can be triggered under certain inputs.
We further study a popular Kalman-Filter based fusion method \cite{fusionmathwork, attackmathworkkalmanfilter}, and use it to replace \op's default fusion method to evaluate it in the context of an entire system.





\subsection{\new{Causality Analysis}}
Over the recent years, causality analysis has gained popularity on interpreting machine learning models\cite{nncausal18, nncausal19}. Compared with traditional methods, causal approaches identify causes and effects of a model’s components and thus facilitates reasoning over its decisions. In the current work, we apply causality analysis to define \adas errors that are caused by the fusion method.

We first provide some relevant definitions and notations, most of which are from \cite{causalitydef15}. In causality analysis, the world is described by variables and their values. Some variables may have a causal influence on others. The influence is modeled by a set
of \emph{structural equations}. The variables are split into two sets: \emph{the exogenous variables}, whose values are determined by factors outside the model, and \emph{the endogenous variables}, whose values are ultimately determined by the exogenous variables. In our context, exogenous variables can be a user specified test design for an \adas (e.g., testing the \adas for a left turn at a signalized intersection scenario), the endogenous variables can consist of the configuration for the \adas under test (e.g., the ego car's target speed), the concrete scenario (e.g., the number and locations of the NPC vehicles), and the final test results (e.g., if a collision happen).

Formally, a causal model $M$ is a pair $(S,F)$. 
$S$ is called "signature" and is a triplet $(U,V,R)$. Among them, $U$ is a set of exogenous variables, $V$ is a set of endogenous variables, and $R$ associates with every variable $Y\in U\cup V$ a nonempty set $R(Y)$ of possible values for $Y$. 
$F$ defines a set of modifiable structural equations relating the values of the variables. It associates with each endogenous variable $X\in V$ a function denoted $F_X$ such that $F_X:(\times_{L \in U} R(L)) \times (\times_{N \in V-{X}} R(N)) \rightarrow R(X)$ meaning $F_X$ determines the value of $X$ given the values of all the other variables in $U\cup V$.
% Setting the value of some variable $X$ to $x$ in a causal model $M=(S,F)$ results in a new causal model, denoted $M_{X\leftarrow x}$ which is identical to $M$ except that the equation for $X$ in $F$ is replaced by $X=x$.

Given a signature $S=(U,V,R)$, a primitive event is a formula of the form $X=x$, for $X\in V$ and $x\in R(X)$. 
A causal formula (over $S$) is one of the form $[Y_1\leftarrow y_1,...,Y_k\leftarrow y_k]\phi$, where $\phi$ is a boolean combination of primitive events, $Y_1,...,Y_k$ are distinct variables in $V$, and $y_i\in R(Y_i)$. 
We abbreviate it as $[\overrightarrow{Y}\leftarrow\overrightarrow{y}]\phi$. This says $\phi$ holds if $\overrightarrow{Y}$ were set to $\overrightarrow{y}$. 
We further denote $(M,\overrightarrow{u})\models\phi$ if the causal formula $\phi$ is true in causal model $M$ given context $U=\overrightarrow{u}$. $(M,\overrightarrow{u})\models(X=x)$ if the variable $X$ has value $x$ in the unique solution to the equations in $M$ given context $\overrightarrow{u}$.

The definition of causality is defined relative to a model $M$ and a context $\overrightarrow{u}$. In particular,
\begin{defi}
$\overrightarrow{X}=\overrightarrow{x}$ is an actual cause of $\phi$ in $(M,\overrightarrow{u})$ if the following three conditions hold: \\
AC1. $(M,\overrightarrow{u})\models(\overrightarrow{X}=\overrightarrow{x})$ and $(M,\overrightarrow{u})\models\phi$ \\
AC2. There is a partition of $V$ into two disjoint subsets $\overrightarrow{Z}$ and $\overrightarrow{W}$ (so that
$\overrightarrow{Z}\cap \overrightarrow{W}=\emptyset$) with $\overrightarrow{X} \subseteq \overrightarrow{Z}$ and a setting $\overrightarrow{x}'$ of the variables in $\overrightarrow{X}$ such that if $(M,\overrightarrow{u})\models\overrightarrow{W}=\overrightarrow{w}$ then 
\[
(M,\overrightarrow{u})\models[\overrightarrow{X}\leftarrow \overrightarrow{x'}, \overrightarrow{W}\leftarrow \overrightarrow{w}]\neg\phi
\]
AC3. $\overrightarrow{X}$ is minimal; no subset of $\overrightarrow{X}$ satisfies AC1 and AC2.
\end{defi}

In the current work, given an error happens (i.e., $\phi$ holds), we want to determine if it is caused by the fusion method used ($\overrightarrow{X}=\overrightarrow{x}$).



\section{Fusion in \op}
\label{ssec:fusion_op}


In this section, we first introduce the role of fusion in \op, a commercial ADAS that provides the functionality of ACC and ALC. Next, we provide a motivating example of fusion misbehavior inducing accident of \op. We then review the fusion logic in \op (denoted as \original) to explain the accident. We further introduce a Kalman-filter based fusion method, denoted as \mathworkoriginal, as an additional studied \msf.



\subsection{Overview}
\begin{figure}[ht]
\centering
    {\includegraphics[width=0.48\textwidth]{images/FusionFuzz_Fusion_in_OP.pdf}}
\caption{The role of fusion in \op.}
\label{fig:fusion_in_op}
\end{figure} 

Shown in \Cref{fig:fusion_in_op}, the fusion component in \op receives data about the leading vehicles from the camera processing component and the radar processing component. Each leading vehicle data, denoted as {\it \lead}, consists of the relative speed, relative longitudinal and latitudinal distances to the leading vehicle, and the confidence of this prediction (only for camera). The fusion component aggregates all \lead information from the upstream sensor processing modules and outputs an estimation to the longitudinal control component. Finally, the longitudinal control component outputs the decisions for throttle and brake to control the vehicle. Note that the latitudinal control component only relies on camera data so we do not consider accidents due to the auto-driving car driving out of the lane.

\subsection{A Collision Example}

\begin{figure}[ht]
\centering
    % \subfloat[\label{fig:traj_107}]
    % {\includegraphics[width=0.034\textwidth]{images/dist/traj_heatmap_107.pdf}}
    % \vspace{0.2mm}
    \subfloat[
    $t_0$, rel x:\\
    c:13.7m(0.1)\\
    r:19.2m\\
    f:None\\
    gt:None
    \label{fig:op_bicycle_example_1}
    ]
    {\includegraphics[width=0.14\textwidth]{images/dist/town06_op_107/900.jpg}}
    \vspace{0.1mm}
    \subfloat[
    $t_1$, rel x: \\
    c: 11.8m(13.5)\\
    r: 3.9m\\
    f: None\\
    gt: 2.9m
    \label{fig:op_bicycle_example_2}
    ]
    {\includegraphics[width=0.14\textwidth]{images/dist/town06_op_107/1000.jpg}}
    \vspace{0.1mm}
    \subfloat[
    $t_2$,\\
    collision happens.
    \label{fig:op_bicycle_example_3}
    ]
    {\includegraphics[width=0.14\textwidth]{images/dist/town06_op_107/1100.jpg}}

\caption{A collision example. {\it rel x}: relative longitudinal distance to the leading vehicle. {\it c}: the best camera predicted lead with confidence. {\it r}: the best radar predicted lead. {\it f}: the fusion method prediction. {\it gt}: the ground-truth value.}
\label{fig:motivating_example}
\end{figure} 

\Cref{fig:motivating_example} shows an example where the ego car collides with a bicyclist cutting in. At $t_0$(\Cref{fig:op_bicycle_example_1}), no leading vehicle exists. At $t_1$(\Cref{fig:op_bicycle_example_2}), the bicyclist on the right trying to cut in. While radar predicted lead is close to the ground-truth, the camera ignores the bicyclist. The fusion component trusts the camera so the ego car does not slow down, and finally a collision occurs at $t_2$(\Cref{fig:op_bicycle_example_3}). This example shows an accident caused by a wrong result from the fusion component. But how could the problem happen? 


\subsection{The Internal Logic of Fusion Methods}
\label{ssec:msf_logic}


\noindent\textbf{\original: Heuristic Rule-based Fusion.}
\Cref{fig:fusion_logic_in_op} shows the logic flow of the \op's fusion method \original. It first checks if the auto-driving car is at a low speed and close to any leading vehicle (\textcircled{1}). If so, the closest radar leads are returned. Otherwise, it checks if the confidence of any camera leads go beyond \new{50\%} (\textcircled{2}). If not, leading vehicles will be considered non-existent. Otherwise, it checks if any radar leads match the camera leads. If so, the best-matching radar leads are returned. Otherwise, the camera leads are returned. This logic explains the failure in \Cref{fig:motivating_example}. In particular, due to \textcircled{2} in \Cref{fig:fusion_logic_original}, no leading vehicle is considered existent at $t_1$ so the ego car accelerates until hitting the bicyclist.
\begin{figure}[ht]
\centering
    \subfloat[\original\label{fig:fusion_logic_in_op}]
    {\includegraphics[width=0.24\textwidth]{images/FusionFuzz_OP_fusion_logic.pdf}\label{fig:fusion_logic_original}}
    \subfloat[\mathworkoriginal\label{fig:fusion_logic_in_mathwork}]
    {\includegraphics[width=0.24\textwidth]{images/FusionFuzz_Mathwork_fusion_logic.pdf}\label{fig:fusion_logic_mathworkoriginal}}
\caption{Fusion logic of (a)\original and (b)\mathworkoriginal. C denotes camera and R denotes radar. Green, orange, blue, red, and purple denote input, output, decision, processing, and stored data over generations, respectively.}
\label{fig:fusion_logic}
\end{figure}

\noindent\textbf{\mathworkoriginal: Kalman-Filter Based Fusion.}
Note that various fusion methods are available in addition to the \original.  
\Cref{fig:fusion_logic_in_mathwork} shows the logic of \mathworkoriginal which is a popular fusion method from Mathwork\cite{fusionmathwork}. It starts with the camera-predicted lane to filter out cluttered (i.e. stationary outside the auto-driving car's lane) radar leads in \textcircled{1}. Then, it groups together camera leads and uncluttered radar leads, and matches them with tracked objects from last generation in \textcircled{2}. Tracked objects are then updated.
% \ez{what next step? tracking component for the next generation?}
Finally, matched tracked objects within the current lane are ranked according to their relative longitudinal distances in \textcircled{3} and the data of the closest two leads are returned.
% In this work, we also include \mathworkoriginal fusion method for the evaluation.




% \zs{Give a preliminary/brief categorization (ORIGINAL and MATHWORK) of \bugs based on root causes after showing the examples could be better?}









% An example of \bugs found for \op: the ego car collides with a leading car in the same lane trying to change lane. (a) at $t_0$, fusion component gives correct prediction. (b) at $t_1$, fusion component gives wrong prediction although radar component gives correct prediction. (c) at $t_2$, collision happens. (d) at $t_2'$ collision does not happen since \best fusion is used starting $t_0$.








% According to the levels of Driving Automation chart by the engineering group SAE International \cite{AVlevelchart}, there are six levels of automation ranging from level 0 to level 5. When researchers, practitioners and the general public argue about when self-driving will really be widely deployed, they usually refer to level 4. In contrast, many modern vehicles have already support level 2 of automation which typically provides the functionality like adaptive cruise control, lane-centering and emergency braking. 




% Thus, Waymo conducted simulation testing for more than 15 billion miles in simulation over the years. For efficiently finding corner cases, a good testing strategy is needed to reduce computational cost


% According to the levels of Driving Automation chart by the engineering group SAE International \cite{AVlevelchart}, there are six levels of automation ranging from level 0 to level 5. When Researchers, practitioners and the general public argue about when self-driving will really be widely deployed, they usually refer to level 4. In contrast, many modern vehicles have already support level 2 of automation which typically provides the functionality like adaptive cruise control, lane-centering and emergency braking.

% In a recent COMMA CON, Harald Schäfer, the CTO of COMMA AI which is the company builds \op, a widely used level-2 \adas, mentioned that the one major limiting factor of reaching the next milestone is to build the infrastructure to test how well the model predict in paper form.





==> body/3_examples.tex <==










% \subsection{Interaction between ego car and world}
% We denote the world update function as the ego car's behavior denoted as $f$,

% At time $i$, denote world state as $S_i$ and ego car's state as $s_i$.
% The process is as the following:
% 1.$WS_i$

% Denote the world as $W$, the ego car behavior can 

% Fusion error is defined 
% causal dependence
% The definition draws from counter-factual 
% "Where c and e are two distinct actual events, e causally depends on c if and only if, if c were not to occur e would not occur."





% References:
% 1.General Problem / System / Scenario Formulation
% Testing Vision-Based Control Systems Using LearnableEvolutionary Algorithms
% AV-FUZZER: Finding Safety Violations inAutonomous Driving Systems
% Testing Autonomous Cars for Feature Interaction Failures usingMany-Objective Search

% 2.Fusion Related Work
% Exploring Adversarial Robustness of Multi-sensor Perception Systemsin Self Driving
% Invisible for both Camera and LiDAR: Security ofMulti-Sensor Fusion based Perception inAutonomous Driving Under Physical-World Attacks
% Drift with Devil: Security of Multi-Sensor Fusion based Localization inHigh-Level Autonomous Driving under GPS Spoofing

\section{Overview} %The Fusion Error}
\label{sec:overview}

The focus of the current paper is to find errors caused by the fusion method used. Fusion errors occur when (i) two sensors' outputs differ significantly, and then (ii) the logic of fusion (i.e., merging the sensor outputs) prioritizes the faulty outputs. To simulate such errors, \tool first efficiently searches (a.k.a. fuzz) the given driving environment to find  \specificss that maximize the differences between the involved sensors and thus, lead to accidents (see~\Cref{subsec:fuzz}). \tool then changes the existing fusion logic with alternative ones and check whether the updated logic can avoid the  simulated crashes (see~\Cref{subsec:causality}). If a collision is avoidable with alternative fusion logic, \tool concludes that original fusion logic was erroneous.  This section summarizes these steps.
%We will start by defining the fusion errors.
%The focus of the current paper is to find errors caused by the fusion method used. Finding such error involves two steps: 1.how to generate the ground-truth for such errors. 2.how to find such errors.

\subsection{Defining Fusion Errors}
%\subsection{Definition}
\label{subsec:definition}

%We first provide the definition of a \bug. After that we justify the definition using causality analysis. 
%We deem that 
Our goal is to simulate errors, i.e., accidents, that may happen due to incorrect fusion logic.
A \bug should have the following two properties: % as to be critical and fusion-induced. 

\begin{itemize}[leftmargin=*]
    \item {\em Critical}: A simulation should witness a {\it collision} of the ego car. Since only the longitudinal control module in \op relies on fusion, we don't consider the accidents likely caused by the misbehaviors of the latitudinal control. For example, we ignore scenarios in which \op drives out of its current lane.
    
    %Instead, we mainly focus on the collisions within the ego car's current lane}. 
    % ~\ziyuan{What does longitudinal control have to do with collision?}
    
    \item {\em Fusion-induced}: The collision should be caused by the misbehavior of the fusion component. In other words, if the rest of the \adas system and environment behave as it is, and we had a correct implementation of sensor fusion, the collision would not be observed. 
\end{itemize}


% \subsubsection{Critical}

% A simulation should witness an {\it accident} of the ego car. Since only the longitudinal control module in \op relies on fusion, we focus on the collision accidents.

% \subsubsection{Avoidable} %a simulation results in an {\it error} if it results in an accident and the accident is avoidable. 
% The happened accident should be avoidable. 
% % We focus on the cases where the ego car has enough time to stop before the collision. Besides, 
% The collision must happen within the field of view of the ego car so \op's camera is able to see the NPC (Non-player character) vehicle. Besides, the ego car must be non-stationary when the collision happens. An example of an accident not being avoidable is when an NPC vehicle accelerates to collide with the end of the ego car. Such accidents cannot be avoided by only improving the \adas so they are not our focus in the current work.

% \subsubsection{Fusion-induced} 
% The critical simulation collision should be causally induced by the misbehavior of the fusion component.
% Since the ego car is a real-time dynamic system and an error occurs only after many time steps of simulation, it is not easy to determine if an error is causally induced by the fusion module.

% In the counterfactual theories of causation\cite{sep-causation-counterfactual}, causal dependence is: {\it "Where c and e are two distinct actual events, e causally depends on c if and only if, if c were not to occur e would not occur."}
% However, such a definition might suffer from minimality and multiple causes as pointed in \cite{causalitydef15}.

% Inspired by it, we make the formal definition:
% To this end, we define the fusion error as:

% \begin{defi}
% An error of the ego car is considered a \bug if, given everything else is kept the same, the error would not occur once the \emph{best-sensor fusion} logic is used during the \emph{pre-crash} period in a counterfactual world.
% \end{defi}


\begin{figure}[ht]
\centering
    {\includegraphics[width=0.48\textwidth]{images/FusionFuzz_Fusion_Error_Definition.pdf}}
\caption{An illustration of pre-crash period and \bug.}
\label{fig:errordefinition_of_fusionfuzz}
\end{figure}

% \Cref{fig:errordefinition_of_fusionfuzz} illustrates such a \bug. At \textcircled{1}, a simulation starts and \op is engaged. The simulation enters the pre-crash period (i.e., the $m$ seconds before an accident) at \textcircled{2} and finally a collision happens at \textcircled{3}. If the best-sensor fusion is used from \textcircled{2} onward, in the counter-factual world, no collision happens at \textcircled{3'}. The main reason we only replace during the pre-crash period is that empirically the misbehavior of the fusion method usually happen towards the end of a simulation.

\Cref{fig:errordefinition_of_fusionfuzz} illustrates such a \bug. At time \textcircled{1}, a simulation starts and \op is engaged. The simulation enters the pre-crash period (i.e., the $m$ seconds before an accident \new{during which it starts to misbehave}) at time \textcircled{2} and finally, a collision happens at \textcircled{3}. If \new{a better fusion method} is used from time \textcircled{2} onward, in the counter-factual world, no collision happens (at time \textcircled{3'~}). 

%Such fusion errors may occur when given the same environment two sensors defer significantly in their output. 


%\subsection{Fuzzing to Simulate Fusion Errors}
\subsection{Simulating Errors with Fusion Fuzzing}
\label{subsec:fuzz}

 Fusion errors may occur when two sensors defer significantly in their outputs given the same input environment.
To find such errors efficiently, we apply an evolutionary-based fuzzing algorithm that searches for the scenarios in which \bugs are likely to happen. The main difference between our method and previous work \cite{avfuzzer, covavfuzz, nsga2nn, testing_vision18, autofuzz21} is that we focus on \bugs rather than the general errors. Accordingly, our fitness function contains a specially designed objective $F_{fusion}$. 

Given a \specifics $x$, the fitness function is a weighted sum of multiple objective functions $\textbf{F}(x)=c_i \sum \textbf{F}_i(x)$, where $\textbf{F}_i$ is an objective and $c_i$ is the weight. 

Recall that \bugs have two important properties (i.e. critical, and fusion-induced), so we design the objective functions accordingly. 
%Note that "avoidable" cannot be explicitly designed as an objective function to optimized for so we are not considering it here. 
For the {\it critical} aspect, we adopt the safety potential objective used in \cite{avfuzzer}. It represents the minimum value of the distance between the ego car and the leading vehicle, subtracted by the ego car's minimum stopping distance. We denote it as $\textbf{F}_{d}(x)$ for the scenario $x$. We further use a boolean objective function which is true only if a collision happens. We denote this objective function as $\textbf{F}_{\textrm{error}}$.

% \noindent\textbf{Avoidable}: 
% For the {\it avoidable} aspect, we use a boolean objective function which is true only if (1) a collision happens; (2) the collided object is within the view of the ego car; and (3) the ego car is not stationary at the time the collision happens. We denote this objective function as $\textbf{F}_{\textrm{error}}$. Note this objective also contributes to the critical aspect.

For the {\it fusion-induced} aspect, we introduce a proxy objective. According to our definition of a \bug, we cannot determine if an error is a \bug without re-running the simulation with the best-sensor fusion. Since the rerunning is costly for the fuzzing process, we use a proxy objective $\textbf{F}_{\textrm{fusion}}$ instead. It is the percentage of the number of frames in which the fusion predicted \lead having large deviation from the ground-truth \lead, while at least one predicted \lead from upstream sensor processing modules is close to the ground-truth \lead:
\begin{equation}
\begin{split}
    \textbf{F}_{\textrm{fusion}}(x) = \frac{1}{|\mathbf{P}|}\times 
    &|\{ i |~~\exists~k \in \mathbf{K} \textrm{ s.t. } ||\hat{s}_{ik}-y_{i}||_1 <th \\
    & \textrm{ and } ||\hat{y}_{i}-y_{i}||_1 >th \textrm{ and } i \in \mathbf{P}\}|
\end{split}
\end{equation}
where $\mathbf{P}$ is a set of indices of the frames during the pre-crash period, \new{$\mathbf{K}$ is a set of indices of the sensors}, $\hat{s}_{ik}$ is a predicted lead by sensor $k$ at time frame $i$, $\hat{y}_i$ is the predicted \lead by the fusion component, $y_i$ is the ground-truth \lead and $th$ is an error threshold. Note each lead variable here is three-dimensional (i.e. relative longitudinal distance, relative latitudinal distance, and relative speed) and each of them is scaled down (by $4$m, $1$m, and $2.5$m/s, respectively\new{, which are chosen based on domain knowledge as well as the empirical  observations}). $th$ is set to $3$ by default \new{meaning the prediction at a frame is considered accurate only when none of the three predictions has large deviations from the ground-truth.}


Finally, putting the above objectives together, we obtain the fitness function:
\begin{equation}
    \textbf{F}(x) = c_{\textrm{error}} \textbf{F}_{\textrm{error}}(x) + c_{d} \textbf{F}_{d}(x) + c_{\textrm{fusion}} \textbf{F}_{\textrm{fusion}}(x)
\end{equation}
Note that the objective functions are all standardized and normalized. 





% \subsection{Justifying Fusion Errors}
% \label{subsec:causality}

\subsection{Analyzing Errors with Counterfactual Fusion Logic}
\label{subsec:causality}

We next justify when an error is a \bug, the error must be caused by the fusion method used.


In the theory of causality analysis, in order to attribute the cause of an event (collision) to another event (the fusion method used), Definition 3 must be satisfied.
The issue then becomes how our definition can satisfy the conditions specified in Definition 3.

In order to reason about the influence of the fusion method used as well as other things during the simulation, we construct a causal graph (\Cref{fig:causal_graph}) based on domain knowledge and map the variables in the causal graph to the relevant variables in Definition 3. 

% We make an assumption that all the variables that can influence the occurrence of a collision have been included in our graph.

% and apply an intervention to remove uncontrollable exogenous variables, and show how the causality of the fusion method on the occurrence of an collision can be determined via finding a fusion method that helps avoiding the initial collision. Next, we propose a fusion method and identify causality based on its test results. Finally, we propose a practical way to efficiently check the causality in practice.

% Following \cite{causalitydef15}, 

% Using domain knowledge, we construct a causal graph for the simulation as shown in \Cref{fig:causal_graph}. 
In particular, the exogenous variables $U$ include test design and the state of the system running simulation (e.g., real-time CPU workload, memory usage, etc.). 
Test design determines scenario to test, simulator configurations (including communication configuration and other configuration), and \op configurations (communication configuration, fusion method, and other configuration). 
Another endogenous variable "communication latency" represents the real-time latency of the communication between the simulator and \op. It is influenced by the configurations of simulator and \op, as well as the system state.
Finally, scenario, simulator configuration, \op configuration, and the communication latency jointly determine the occurrence of a collision in the simulation. 

We define $\overrightarrow{X}$ to be the fusion method, $\overrightarrow{Y}$ to be a boolean variable representing the occurrence of a collision, and $\phi=\overrightarrow{Y}$. Given a collision happens (i.e., $\phi$ holds), we want to determine if the fusion method ($\overrightarrow{X}=\overrightarrow{x}$) is the actual cause. $\overrightarrow{Z}$ is supposed to include $\overrightarrow{X}$ and the variables influenced by it. In our case, it is the union of $\overrightarrow{X}$ and $\overrightarrow{Y}$. $\overrightarrow{W}$ includes all the endogenous variables that are not in $\overrightarrow{Z}$.

Since $\overrightarrow{X}$ only consists of one variable, the minimality condition AC3 is satisfied automatically. Given a collision scenario (i.e., $\phi$ is true), AC1 is also trivially satisfied with the fusion method $\overrightarrow{x}$ used during the collision.

Now the issue comes to how to achieve AC2. Based on its definition, we need to be able to control the exogenous variables $U$ as well as the endogenous variables $\overrightarrow{W}$, and find another fusion method $x'$ such that $\phi$ will not hold. 
However, we cannot control the system state variable in practice. To address it, we set the communication configurations of the simulator and the \op to be deterministic and synchronous (see \Cref{sec:adaption_of_openpilot} for details). The change eliminates the influence of the communication latency on the occurrence of a collision and thus block the influence of the system state. Given the causal graph, if we keep all the context $\overrightarrow{w}$ and test design ($\overrightarrow{u}$) the same as in the initial collision scenario, while only changing the fusion method, if the collision does not happen any more, AC2 is satisfied and we can say that the fusion method causes the collision.


\begin{figure}[ht]
\centering
    {\includegraphics[width=0.4\textwidth]{images/causal_graph.pdf}}
\caption{An illustration of the causal graph with intervention.}
\label{fig:causal_graph}
\end{figure} 

\noindent\textbf{Approximate the Causality}
The next step is to find a fusion method $x'$, if it exists, such that in the counterfactual world (where everything else is kept the same except the fusion method) the collision can be avoided by letting $\overrightarrow{X}=x'$. Since running high-fidelity simulation is costly, if the fusion method causes the collision, we want to use the smallest number of simulations to find it. 
Additionally, the fusion method $x'$ should possess other properties like being realistic and functional. Being realistic means that it should not have extra knowledge (e.g., the ground-truth of the locations of the NPC vehicles) beyond what it receives from the upstream sensor modules. Being functional means it should be good enough to enable the ego car to finish the original task. 
A counter-example is if the fusion method always false positively report the presence of a stationary NPC vehicle ahead and leads the ego car to be stationary all the time. Collision can be avoided in this case since the ego car does not move at all but the original task is not completed neither. 

To better illustrate this, we define three different classes of fusion methods. Given everything else is kept the same, \emph{collision fusion class} and \emph{non-collision fusion class} consist of the fusion methods that lead to and avoid the collision, respectively. \emph{Realistic \& functional class} consists of fusion methods which are both realistic and functional. If an error is caused by the fusion method and can be fixed by changing it to a realistic and functional fusion method, there should be an intersection between non-collision fusion and realistic \& functional fusion as shown in \Cref{fig:fusion_replacement}(a) and \Cref{fig:fusion_replacement}(c). 
Otherwise, there should be no intersection between the two and the realistic \& functional fusion class should be a subset of the collision fusion class as shown \Cref{fig:fusion_replacement}(b). 
The initial fusion method should fall into the intersection of the collision fusion class and the realistic \& functional fusion class since a collision happens and it is reasonable to assume the initial fusion method (\original or \mathworkoriginal) is realistic and functional. 

% This also relates to metamorphic testing \cite{metamorphic}. All the realistic and functional fusion methods that do not lead to collision are metamorphic while all the others are metamorphic.



\begin{figure*}[ht]
\centering
    \subfloat[True Positive\label{fig:fusion_replacement_a}]
    {\includegraphics[width=0.32\textwidth]{images/fusion_replacement_a.pdf}}
   ~
    \subfloat[True Negative\label{fig:fusion_replacement_b}]
    {\includegraphics[width=0.32\textwidth]{images/fusion_replacement_b.pdf}}
    ~
    \subfloat[False Negative\label{fig:fusion_replacement_c}]
    {\includegraphics[width=0.32\textwidth]{images/fusion_replacement_c.pdf}}
    
\caption{An illustration of three situations of replacing the fusion method.}
\label{fig:fusion_replacement}
\end{figure*}


In the current work, we only run one additional simulation for each found collision. In particular, we let $x'$ be a fusion method called \emph{best-sensor fusion}, which always selects the sensor prediction that is closest to the ground-truth. Note that this fusion method is an oracle fusion method since in reality we won't be able to know the ground-truth. 
However, this fusion method serves a good proxy. 
First, it is realistic. Although we leverage ground-truth for it, in reality, a fusion method might potentially achieve the best-sensor fusion method's output which is the most reliable upstream sensor's prediction. 
Second, it is functional since the downstream modules are usually optimized with the assumption that the fusion method can provide a relatively reliable prediction and thus should be able to finish the original cruising task. Third, if \emph{best-sensor fusion} cannot help avoid the initial collision after the replacement, there is a high possibility that the collision is not due to the fusion method. The reason is that this fusion method already picks the best sensor prediction and it is reasonable to assume that the downstream modules are more likely to perform better given it compared with a fusion method providing a less accurate prediction.

Thus, best-sensor fusion serves as a proxy to check if there is an intersection between realistic \& functional fusion and non-collision fusion. If best-sensor fusion can help avoid the collision, the error will be considered \emph{fusion-induced}. Otherwise, it is considered \emph{not fusion-induced}.
There are three situations: (a)the error is caused by the fusion method and the best-sensor fusion falls into non-collision fusion. (b)the error is not caused by the fusion method and the best-sensor fusion does not fall into non-collision fusion. (c) the error is caused by the fusion method and the best-sensor fusion does not fall into non-collision fusion. (a) and (b) are the desirable true positive and true negative cases since the causation of the fusion method is consistent with the collision results of the best-sensor fusion method, while (c) is the false negative case. It also should be noted that there is no false positive case since if best-sensor fusion helps avoiding the collision, according to our reasoning earlier, the causation must hold. The implication is that a fusion-induced error is an error caused by the fusion method but the reverse does not always hold. 







\subsection{Counting Fusion Errors}
\label{sec:error_counting}
We design the principles for counting distinct \bugs in this section. Note that error counting in simulation-based testing remains an open challenge. Related works \cite{paracosm, testing_vision18} consider two errors being different if the \specificss are different. This definition tends to over-count similar errors when the search space is high-dimensional. %For example, two \bugs is considered different if the type of a never seen NPC vehicle having no interaction with other NPCs is changed. 
Another approach manually judges errors with human efforts \cite{avfuzzer}. Such way is subjective and time-consuming when the number of errors grows up. 

Inspired by the location trajectory coverage metric \cite{covavfuzz}, we also consider the ego car's state (in particular, position and speed) during the simulation rather than the input space variables or human judgement. 
% We report this counting number as the metric to compare the fuzzing methods and give examples to justify this definition.  In particular, we conduct counting based on "spatial-speed trajectory coverage". 
We split the pieces of the lane that ego car drives on into $s$ intervals and the ego car's allowed speed range into $l$ intervals to get a two-dimensional coverage plane with dimensions $\mathbf{1}^{s\times l}$. During the simulation, the ego car's real-time location and speed are recorded at 2Hz. The recorded location-speed data points are then mapped to their corresponding "cells" on the coverage plane. Given all the data points mapped into the cells having the same road interval, their average speed is taken, the corresponding speed-road cell is considered "covered", and the corresponding field on the coverage plane is assigned $1$. Note a simulation's final trajectory representation can have at most $s$ non-zero fields although it has $s\times l$ fields in total.

% \zs{A vector is usually represented by a bold letter or with an arrow on top. There are a lot of regular font "traj"s which are not words or symbols. Use trajectory} 
We denote the trajectory vector associated with the simulation run for a specification $x$ to be $\mathbf{R}(x)$ and define:
\begin{defi}
Two \bugs for the simulations runs on specifications $x_1$ and $x_2$ are considered distinct if $\vert \vert \mathbf{R}(x_1)-\mathbf{R}(x_2)\vert \vert_0 > 0$.
\label{errors_count}
\end{defi}

\begin{figure}[ht]
\centering
    \subfloat[\label{fig:traj_357}]
    {\includegraphics[width=0.034\textwidth]{images/dist/traj_heatmap_357.pdf}}
    \vspace{0.2mm}
    \subfloat[$time_0$]
    {\includegraphics[width=0.14\textwidth]{images/dist/town06_op_357_0/900.jpg}}
    \vspace{0.1mm}
    \subfloat[$time_1$]
    {\includegraphics[width=0.14\textwidth]{images/dist/town06_op_357_0/1000.jpg}}
    \vspace{0.1mm}
    \subfloat[$time_2$]
    {\includegraphics[width=0.14\textwidth]{images/dist/town06_op_357_0/1100.jpg}}

    \subfloat[\label{fig:traj_445}]
    {\includegraphics[width=0.034\textwidth]{images/dist/traj_heatmap_445.pdf}}
    \vspace{0.2mm}
    \subfloat[$time_0$]
    {\includegraphics[width=0.14\textwidth]{images/dist/town06_op_445_30/2100.jpg}}
    \vspace{0.1mm}
    \subfloat[$time_1$]
    {\includegraphics[width=0.14\textwidth]{images/dist/town06_op_445_30/2175.jpg}}
    \vspace{0.1mm}
    \subfloat[$time_2$]
    {\includegraphics[width=0.14\textwidth]{images/dist/town06_op_445_30/2250.jpg}}
\caption{Examples of two \bugs with different trajectories. (a) and (e) show speed-location coverage where the x-axis is speed and y axis is the road interval.}
\label{fig:traj_demo}
\end{figure} 


To demonstrate this error counting approach, we show two \bugs %(found by \tool on \original in \Sa) under the \Cref{fig:motivating_example} scenario 
with different trajectories in \Cref{fig:traj_demo}. 
In both \Cref{fig:motivating_example} and the first row of \Cref{fig:traj_demo}, the ego car hits a bicyclist cutting in from the right lane. The difference is only that the yellow car on the left lane has different behaviors across the two runs. However, the yellow car does not influence the ego car's behavior. Hence, the two simulation runs have the same trajectory coverage (ref. \Cref{fig:traj_357}). 
By contrast, the other \bug on the second row of \Cref{fig:traj_demo} has a different trajectory (ref. \Cref{fig:traj_445}) that the ego car in high speed collides with a motorcycle at a location close to the destination. This example illustrates the necessity of counting \bugs upon \Cref{errors_count}.



% We further manually classify these distinct \bugs based on human judgement as different categories according to root cause and report the number of distinct \bugs categories found by each fuzzing method.






\subsection{\new{Background: Causality Analysis}}
Over the recent years, causality analysis has gained popularity on interpreting machine learning models\cite{nncausal18, nncausal19}. Compared with traditional methods, causal approaches identify causes and effects of a model’s components and thus facilitates reasoning over its decisions. In the current work, we apply causality analysis to justify the defined \bugs are indeed \adas errors caused by the fusion method.

In causality analysis, the world is described by variables and their values. Some variables may have a causal influence on others. The influence is modeled by a set of \emph{structural equations}. The variables are split into two sets: \emph{the exogenous variables}, whose values are determined by factors outside the model, and \emph{the endogenous variables}, whose values are ultimately determined by the exogenous variables. In our context, exogenous variables can be a user specified test design for an \adas (e.g., testing the \adas for a left turn at a signalized intersection scenario), the endogenous variables can consist of the configuration for the \adas under test (e.g., the ego car's target speed), the concrete scenario (e.g., the number and locations of the NPC vehicles), and the final test results (e.g., if a collision happen).

Formally, a causal model $M$ is a pair $(S,F)$. 
$S$ is called "signature" and is a triplet $(U,V,R)$. Among them, $U$ is a set of exogenous variables, $V$ is a set of endogenous variables, and $R$ associates with every variable $Y\in U\cup V$ a nonempty set $R(Y)$ of possible values for $Y$. 
$F$ defines a set of modifiable structural equations relating the values of the variables. 

Given a signature $S=(U,V,R)$, a primitive event is a formula of the form $X=x$, for $X\in V$ and $x\in R(X)$. 
A causal formula (over $S$) is one of the form 
% $[Y_1\leftarrow y_1,...,Y_k\leftarrow y_k]\phi$, where $\phi$ is a boolean combination of primitive events, $Y_1,...,Y_k$ are distinct variables in $V$, and $y_i\in R(Y_i)$. 
% We abbreviate it as 
$[\overrightarrow{Y}\leftarrow\overrightarrow{y}]\phi$, where $\overrightarrow{Y}$ is a subset of variables in $V$ and $\phi$ is a boolean combination of primitive events. This says $\phi$ holds if $\overrightarrow{Y}$ were set to $\overrightarrow{y}$. 
We further denote $(M,\overrightarrow{u})\models\phi$ if the causal formula $\phi$ is true in causal model $M$ given context $U=\overrightarrow{u}$. $(M,\overrightarrow{u})\models(X=x)$ if the variable $X$ has value $x$ in the unique solution to the equations in $M$ given context $\overrightarrow{u}$.

% The definition of causality is defined relative to a model $M$ and a context $\overrightarrow{u}$. 
We next provide the definition of causality.
\begin{defi}
$\overrightarrow{X}=\overrightarrow{x}$ is an actual cause of $\phi$ in $(M,\overrightarrow{u})$ if the following three conditions hold: \\
AC1. $(M,\overrightarrow{u})\models(\overrightarrow{X}=\overrightarrow{x})$ and $(M,\overrightarrow{u})\models\phi$ \\
AC2. There is a partition of $V$ into two disjoint subsets $\overrightarrow{Z}$ and $\overrightarrow{W}$ (so that
$\overrightarrow{Z}\cap \overrightarrow{W}=\emptyset$) with $\overrightarrow{X} \subseteq \overrightarrow{Z}$ and a setting $\overrightarrow{x}'$ of the variables in $\overrightarrow{X}$ such that if $(M,\overrightarrow{u})\models(\overrightarrow{W}=\overrightarrow{w})$ then 
\[
(M,\overrightarrow{u})\models[\overrightarrow{X}\leftarrow \overrightarrow{x'}, \overrightarrow{W}\leftarrow \overrightarrow{w}]\neg\phi
\]
AC3. $\overrightarrow{X}$ is minimal; no subset of $\overrightarrow{X}$ satisfies AC1 and AC2.
\end{defi}

AC1 means both $\overrightarrow{X}=\overrightarrow{x}$ and $\phi$ happen. 
AC3 is a minimality condition. It makes sure only elements within $\overrightarrow{X}$ that are essential are considered as part of a cause. 
Without AC3, if studying hard causes good grade then so is studying hard and being tall.
AC2 essentially says when keeping everything else (except $\overrightarrow{X}$ and those influenced by it) exactly the same, there is a $\overrightarrow{x}'$ such that it can make $\phi$ does not hold.

In the current work, given an error happens (i.e., $\phi$ holds), we want to determine if the fusion method ($\overrightarrow{X}=\overrightarrow{x}$) is the actual cause. To achieve this, we want to identify scenarios such that AC1-AC3 are all satisfied. In fact, our defined \bugs satisfy them.





% In causality analysis, the world is described by variables and their values. Some variables may have a causal influence on others. The influence is modeled by a set
% of \emph{structural equations}. The variables are split into two sets: \emph{the exogenous variables}, whose values are determined by factors outside the model, and \emph{the endogenous variables}, whose values are ultimately determined by the exogenous variables. In our context, exogenous variables can be a user specified test design for an \adas (e.g., testing the \adas for a left turn at a signalized intersection scenario), the endogenous variables can consist of the configuration for the \adas under test (e.g., the ego car's target speed), the concrete scenario (e.g., the number and locations of the NPC vehicles), and the final test results (e.g., if a collision happen).

% Formally, a causal model $M$ is a pair $(S,F)$. 
% $S$ is called "signature" and is a triplet $(U,V,R)$. Among them, $U$ is a set of exogenous variables, $V$ is a set of endogenous variables, and $R$ associates with every variable $Y\in U\cup V$ a nonempty set $R(Y)$ of possible values for $Y$. 
% $F$ defines a set of modifiable structural equations relating the values of the variables. 
% % It associates with each endogenous variable $X\in V$ a function denoted $F_X$ such that $F_X:(\times_{L \in U} R(L)) \times (\times_{N \in V-{X}} R(N)) \rightarrow R(X)$ meaning $F_X$ determines the value of $X$ given the values of all the other variables in $U\cup V$.
% % Setting the value of some variable $X$ to $x$ in a causal model $M=(S,F)$ results in a new causal model, denoted $M_{X\leftarrow x}$ which is identical to $M$ except that the equation for $X$ in $F$ is replaced by $X=x$.

% Given a signature $S=(U,V,R)$, a primitive event is a formula of the form $X=x$, for $X\in V$ and $x\in R(X)$. 
% A causal formula (over $S$) is one of the form $[Y_1\leftarrow y_1,...,Y_k\leftarrow y_k]\phi$, where $\phi$ is a boolean combination of primitive events, $Y_1,...,Y_k$ are distinct variables in $V$, and $y_i\in R(Y_i)$. 
% We abbreviate it as $[\overrightarrow{Y}\leftarrow\overrightarrow{y}]\phi$. This says $\phi$ holds if $\overrightarrow{Y}$ were set to $\overrightarrow{y}$. 
% We further denote $(M,\overrightarrow{u})\models\phi$ if the causal formula $\phi$ is true in causal model $M$ given context $U=\overrightarrow{u}$. $(M,\overrightarrow{u})\models(X=x)$ if the variable $X$ has value $x$ in the unique solution to the equations in $M$ given context $\overrightarrow{u}$.

% The definition of causality is defined relative to a model $M$ and a context $\overrightarrow{u}$. In particular,
% \begin{defi}
% $\overrightarrow{X}=\overrightarrow{x}$ is an actual cause of $\phi$ in $(M,\overrightarrow{u})$ if the following three conditions hold: \\
% AC1. $(M,\overrightarrow{u})\models(\overrightarrow{X}=\overrightarrow{x})$ and $(M,\overrightarrow{u})\models\phi$ \\
% AC2. There is a partition of $V$ into two disjoint subsets $\overrightarrow{Z}$ and $\overrightarrow{W}$ (so that
% $\overrightarrow{Z}\cap \overrightarrow{W}=\emptyset$) with $\overrightarrow{X} \subseteq \overrightarrow{Z}$ and a setting $\overrightarrow{x}'$ of the variables in $\overrightarrow{X}$ such that if $(M,\overrightarrow{u})\models(\overrightarrow{W}=\overrightarrow{w})$ then 
% \[
% (M,\overrightarrow{u})\models[\overrightarrow{X}\leftarrow \overrightarrow{x'}, \overrightarrow{W}\leftarrow \overrightarrow{w}]\neg\phi
% \]
% AC3. $\overrightarrow{X}$ is minimal; no subset of $\overrightarrow{X}$ satisfies AC1 and AC2.
% \end{defi}

% In the current work, given an error happens (i.e., $\phi$ holds), we want to determine if it is caused by the fusion method used ($\overrightarrow{X}=\overrightarrow{x}$).















% Note that the condition in the definition is sufficient but not necessary as we showed earlier in \Cref{fig:fusion_replacement}(c). 

 








==> body/3_examples_backup.tex <==










% \subsection{Interaction between ego car and world}
% We denote the world update function as the ego car's behavior denoted as $f$,

% At time $i$, denote world state as $S_i$ and ego car's state as $s_i$.
% The process is as the following:
% 1.$WS_i$

% Denote the world as $W$, the ego car behavior can 

% Fusion error is defined 
% causal dependence
% The definition draws from counter-factual 
% "Where c and e are two distinct actual events, e causally depends on c if and only if, if c were not to occur e would not occur."





% References:
% 1.General Problem / System / Scenario Formulation
% Testing Vision-Based Control Systems Using LearnableEvolutionary Algorithms
% AV-FUZZER: Finding Safety Violations inAutonomous Driving Systems
% Testing Autonomous Cars for Feature Interaction Failures usingMany-Objective Search

% 2.Fusion Related Work
% Exploring Adversarial Robustness of Multi-sensor Perception Systemsin Self Driving
% Invisible for both Camera and LiDAR: Security ofMulti-Sensor Fusion based Perception inAutonomous Driving Under Physical-World Attacks
% Drift with Devil: Security of Multi-Sensor Fusion based Localization inHigh-Level Autonomous Driving under GPS Spoofing

\section{The Fusion Error}
\new{In this section, we first provide the necessary background of causality analysis. Next, we provide a formal definition of the \bugs using causality analysis and design a way to distinguish them based on trajectory coverage.}


\subsection{\new{Causality Analysis}}
Over the recent years, causality analysis has gained popularity on interpreting machine learning models\cite{nncausal18, nncausal19}. Compared with traditional methods, causal approaches identify causes and effects of a model’s components and thus facilitates reasoning over its decisions. In the current work, we apply causality analysis to define \adas errors that are caused by the fusion method.

We first provide some relevant definitions and notations, most of which are from \cite{causalitydef15}. In causality analysis, the world is described by variables and their values. Some variables may have a causal influence on others. The influence is modeled by a set
of \emph{structural equations}. The variables are split into two sets: \emph{the exogenous variables}, whose values are determined by factors outside the model, and \emph{the endogenous variables}, whose values are ultimately determined by the exogenous variables. In our context, exogenous variables can be a user specified test design for an \adas (e.g., testing the \adas for a left turn at a signalized intersection scenario), the endogenous variables can consist of the configuration for the \adas under test (e.g., the ego car's target speed), the concrete scenario (e.g., the number and locations of the NPC vehicles), and the final test results (e.g., if a collision happen).

Formally, a causal model $M$ is a pair $(S,F)$. 
$S$ is called "signature" and is a triplet $(U,V,R)$. Among them, $U$ is a set of exogenous variables, $V$ is a set of endogenous variables, and $R$ associates with every variable $Y\in U\cup V$ a nonempty set $R(Y)$ of possible values for $Y$. 
$F$ defines a set of modifiable structural equations relating the values of the variables. It associates with each endogenous variable $X\in V$ a function denoted $F_X$ such that $F_X:(\times_{L \in U} R(L)) \times (\times_{N \in V-{X}} R(N)) \rightarrow R(X)$ meaning $F_X$ determines the value of $X$ given the values of all the other variables in $U\cup V$.
% Setting the value of some variable $X$ to $x$ in a causal model $M=(S,F)$ results in a new causal model, denoted $M_{X\leftarrow x}$ which is identical to $M$ except that the equation for $X$ in $F$ is replaced by $X=x$.

Given a signature $S=(U,V,R)$, a primitive event is a formula of the form $X=x$, for $X\in V$ and $x\in R(X)$. 
A causal formula (over $S$) is one of the form $[Y_1\leftarrow y_1,...,Y_k\leftarrow y_k]\phi$, where $\phi$ is a boolean combination of primitive events, $Y_1,...,Y_k$ are distinct variables in $V$, and $y_i\in R(Y_i)$. 
We abbreviate it as $[\overrightarrow{Y}\leftarrow\overrightarrow{y}]\phi$. This says $\phi$ holds if $\overrightarrow{Y}$ were set to $\overrightarrow{y}$. 
We further denote $(M,\overrightarrow{u})\models\phi$ if the causal formula $\phi$ is true in causal model $M$ given context $U=\overrightarrow{u}$. $(M,\overrightarrow{u})\models(X=x)$ if the variable $X$ has value $x$ in the unique solution to the equations in $M$ given context $\overrightarrow{u}$.

The definition of causality is defined relative to a model $M$ and a context $\overrightarrow{u}$. In particular,
\begin{defi}
$\overrightarrow{X}=\overrightarrow{x}$ is an actual cause of $\phi$ in $(M,\overrightarrow{u})$ if the following three conditions hold: \\
AC1. $(M,\overrightarrow{u})\models(\overrightarrow{X}=\overrightarrow{x})$ and $(M,\overrightarrow{u})\models\phi$ \\
AC2. There is a partition of $V$ into two disjoint subsets $\overrightarrow{Z}$ and $\overrightarrow{W}$ (so that
$\overrightarrow{Z}\cap \overrightarrow{W}=\emptyset$) with $\overrightarrow{X} \subseteq \overrightarrow{Z}$ and a setting $\overrightarrow{x}'$ of the variables in $\overrightarrow{X}$ such that if $(M,\overrightarrow{u})\models\overrightarrow{W}=\overrightarrow{w}$ then 
\[
(M,\overrightarrow{u})\models[\overrightarrow{X}\leftarrow \overrightarrow{x'}, \overrightarrow{W}\leftarrow \overrightarrow{w}]\neg\phi
\]
AC3. $\overrightarrow{X}$ is minimal; no subset of $\overrightarrow{X}$ satisfies AC1 and AC2.
\end{defi}

In the current work, given an error happens (i.e., $\phi$ holds), we want to determine if it is caused by the fusion method used ($\overrightarrow{X}=\overrightarrow{x}$).







\subsection{\new{The Definition}}
We deem that a \bug should have two properties as to be critical and fusion-induced. 
% \ez{we first define what type of errors are considered towards fusion errors: ...} 

\subsubsection{Critical}
A simulation should witness an {\it accident} of the ego car. Since only the longitudinal control module in \op relies on fusion, we focus on the collision accidents.

% \subsubsection{Avoidable} %a simulation results in an {\it error} if it results in an accident and the accident is avoidable. 
% The happened accident should be avoidable. 
% % We focus on the cases where the ego car has enough time to stop before the collision. Besides, 
% The collision must happen within the field of view of the ego car so \op's camera is able to see the NPC (Non-player character) vehicle. Besides, the ego car must be non-stationary when the collision happens. An example of an accident not being avoidable is when an NPC vehicle accelerates to collide with the end of the ego car. Such accidents cannot be avoided by only improving the \adas so they are not our focus in the current work.

\subsubsection{Fusion-induced} % a simulation results in a {\it \bug} if it results in an error and the error is  
The critical simulation collision should be causally induced by the misbehavior of the fusion component.
% Since the ego car is a real-time dynamic system and an error occurs only after many time steps of simulation, it is not easy to determine if an error is causally induced by the fusion module. \ez{the last sentence might be removed.}
The challenge is how to identify this causality since a collision might happen due to another cause. To overcome the challenge, we first present the definition of causality proposed in \cite{causalitydef15}. We then construct a causal graph for our context based on domain knowledge and apply an intervention to remove uncontrollable exogenous variables, and show how the causality of the fusion method on the occurrence of an collision can be determined via finding a fusion method that helps avoiding the initial collision. Next, we propose a fusion method and identify causality based on its test results. Finally, we propose a practical way to efficiently check the causality in practice.

\noindent\textbf{Define the Causality}
% Following \cite{causalitydef15}, 

Using domain knowledge, we construct a causal graph for the simulation as shown in \Cref{fig:causal_graph}. We assume that exogenous variables $U$ include test design and the state of the system running simulation (e.g., CPU workload, memory usage, etc.) and all others are endogenous. Test design determines four endogenous variables including \op configuration, simulator configuration, scenario to test, and the fusion method to use. System state along with op configuration and simulator configuration determine an endogenous variable real-time latency within \op and simulator, and between their communications. The aforementioned five endogenous variables collectively determine the occurrence of a collision in the simulation. We let $\overrightarrow{X}$ to be the fusion method,  $\overrightarrow{W}$ consists of \op configuration, real-time latency, simulator configuration, and scenario. We denote $\overrightarrow{Y}$ to be a boolean variable representing the occurrence of a collision. We let $\phi=\overrightarrow{Y}$ such that $\phi$ holds if a collision happens. We also let $\overrightarrow{Z}$ to consist of both $\overrightarrow{X}$ and $\overrightarrow{Y}$.

Since $\overrightarrow{X}$ only consists of one variable, the minimality requirement in AC3 is satisfied automatically. Given a collision scenario (i.e., $\phi$ is true), AC1 is also trivially satisfied with the collision case's test design $\overrightarrow{u}$ and its initial fusion method $\overrightarrow{x}$.

Now the issue comes to how to achieve AC2. Based on its definition, we need to be able to control the exogenous variables $U$ as well as the endogenous variables $\overrightarrow{W}$, and find another fusion method $x'$ that makes $\phi$ do not hold. 
However, we cannot control the system state variable in practice. To address it, we intervene the real-time latency variable by making the simulator and \op deterministic, and their communication synchronous, the details of which can be seen in \Cref{sec:adaption_of_openpilot}. This intervention blocks the influence of system state, and we can thus ignore it. Given the intervened causal graph, if we keep all the context $\overrightarrow{w}$ and test design ($\overrightarrow{u}$) the same as in the initial collision scenario, while only changing the fusion method, if the collision does not happen any more, AC2 is satisfied and we can say that the fusion method causes the collision.


\begin{figure}[ht]
\centering
    {\includegraphics[width=0.4\textwidth]{images/causal_graph.pdf}}
\caption{An illustration of the causal graph with intervention.}
\label{fig:causal_graph}
\end{figure} 

\noindent\textbf{Approximate the Causality}
The next step is to find a fusion method $x'$, if it exists, such that in the counterfactual world (where everything else is kept the same except the fusion method) the collision can be avoided by letting $\overrightarrow{X}=x'$. Since running high-fidelity simulation is costly, if the fusion method causes the collision, we want to use the smallest number of simulations to find it. Additionally, the fusion method $x'$ should possess other properties like being realistic and functional. Being realistic means that it should not have extra knowledge (e.g., the ground-truth of the locations of the NPC vehicles) beyond what it receives from the upstream sensor modules. Being functional means it should be good enough to enable the ego car to finish the original task. A counter-example is if the fusion method always false positively report the presence of a stationary NPC vehicle ahead and leads the ego car to be stationary all the time. Collision can be avoided in this case since the ego car does not move at all but the original task is not completed neither. 

To better illustrate this, we define three different classes of fusion methods. Given everything else is kept the same, \emph{collision fusion class} and \emph{non-collision fusion class} consist of the fusion methods that lead to and avoid the collision, respectively. \emph{Realistic \& functional class} consists of fusion methods which are both realistic and functional. If an error is caused by the fusion method and can be fixed by changing it to a realistic and functional fusion method, there should be an intersection between non-collision fusion and realistic \& functional fusion as shown in \Cref{fig:fusion_replacement}(a) and \Cref{fig:fusion_replacement}(c). Otherwise, there should be no intersection between the two and the realistic \& functional fusion class should be a subset of the collision fusion class as shown \Cref{fig:fusion_replacement}(b). The initial fusion method should fall into the intersection of the collision fusion class and the realistic \& functional fusion class since a collision happens and it is reasonable to assume the initial fusion method (\original or \mathworkoriginal) is realistic and functional. 

% This also relates to metamorphic testing \cite{metamorphic}. All the realistic and functional fusion methods that do not lead to collision are metamorphic while all the others are metamorphic.



\begin{figure*}[ht]
\centering
    \subfloat[True Positive\label{fig:fusion_replacement_a}]
    {\includegraphics[width=0.32\textwidth]{images/fusion_replacement_a.pdf}}
   ~
    \subfloat[True Negative\label{fig:fusion_replacement_b}]
    {\includegraphics[width=0.32\textwidth]{images/fusion_replacement_b.pdf}}
    ~
    \subfloat[False Negative\label{fig:fusion_replacement_c}]
    {\includegraphics[width=0.32\textwidth]{images/fusion_replacement_c.pdf}}
    
\caption{An illustration of three situations of replacing the fusion method.}
\label{fig:fusion_replacement}
\end{figure*}


Since simulation is costly, in the current work, we only run one additional simulation for each found collision. In particular, we let $x'$ be a fusion method called \emph{best-sensor fusion}, which always selects the sensor prediction that is closest to the ground-truth. Note that this fusion method is an oracle fusion method since in reality we won't be able to know the ground-truth. 
However, this fusion method serves a good proxy. 
First, it is realistic. Although we leverage ground-truth for it, in reality, a fusion method might potentially achieve the best-sensor fusion method's output which is the most reliable upstream sensor's prediction rather than the ground-truth. 
Second, it is functional since the downstream modules are usually optimized with the assumption that the fusion method can provide a relatively reliable prediction and thus should be able to finish the original cruising task. Third, if \emph{best-sensor fusion} cannot help avoid the initial collision after the replacement, there is a high possibility that the collision is not due to the fusion method. The reason is that this fusion method already picks the best sensor prediction and it is reasonable to assume that the downstream modules are more likely to perform better given it compared with a fusion method providing a less accurate prediction.

Thus, best-sensor fusion serves as a proxy to check if there is an intersection between realistic \& functional fusion and non-collision fusion. If best-sensor fusion can help avoid the collision, the error will be considered \emph{fusion-induced}. Otherwise, it is considered \emph{not fusion-induced}.
There are three situations: (a)the error is caused by the fusion method and the best-sensor fusion falls into non-collision fusion. (b)the error is not caused by the fusion method and the best-sensor fusion does not fall into non-collision fusion. (c) the error is caused by the fusion method and the best-sensor fusion does not fall into non-collision fusion. (a) and (b) are the desirable true positive and true negative cases since the causation of the fusion method is consistent with the collision results of the best-sensor fusion method, while (c) is the false negative case. It also should be noted that there is no false positive case since if best-sensor fusion helps avoiding the collision, according to our reasoning earlier, the causation must hold. The implication is that the a fusion-induced error is an error caused by the fusion method but the reverse does not always hold. 






% In the counterfactual theories of causation\cite{sep-causation-counterfactual}, causal dependence is: {\it "Where c and e are two distinct actual events, e causally depends on c if and only if, if c were not to occur e would not occur."}
% However, such a definition might suffer from minimality and multiple causes as pointed in \cite{causalitydef15}.

% Inspired by it, we make the formal definition:

\noindent\textbf{Evaluate the Causality}
We next provide a practical definition of \bug in our context. As depicted in Figure~\ref{fig:errordefinition_of_fusionfuzz}, we further denote a {\it pre-crash period} consists of the $m$ seconds before an accident during which the replacement is conducted. The main reason is that the misbehavior of the fusion method usually happen towards the end of a simulation. We define:
\begin{defi}
An error of the ego car is considered a \bug if, given everything else is kept the same, the error would not occur once the \emph{best-sensor fusion} is used during the \emph{pre-crash} period in a counterfactual world.
\end{defi}


\begin{figure}[ht]
\centering
    {\includegraphics[width=0.48\textwidth]{images/FusionFuzz_Fusion_Error_Definition.pdf}}
\caption{An illustration of pre-crash period and \bug.}
\label{fig:errordefinition_of_fusionfuzz}
\end{figure}

\Cref{fig:errordefinition_of_fusionfuzz} illustrates such a \bug. At \textcircled{1}, a simulation starts and \op is engaged. The simulation enters the pre-crash period at \textcircled{2} and finally a collision happens at \textcircled{3}. If the best-sensor fusion is used from \textcircled{2}, in the counter-factual world, no collision happens at \textcircled{3}. 
% Note that the condition in the definition is sufficient but not necessary as we showed earlier in \Cref{fig:fusion_replacement}(c). 

 


\subsection{Error Counting}
\label{sec:error_counting}
We design the principles for counting distinct \bugs in this section. Note that error counting in simulation-based testing remains an open challenge. Related works \cite{paracosm, testing_vision18} consider two errors being different if the \specificss are different. This definition tends to over-count similar errors when the search space is high-dimensional. %For example, two \bugs is considered different if the type of a never seen NPC vehicle having no interaction with other NPCs is changed. 
Another approach manually judges errors with human efforts \cite{avfuzzer}. Such way is subjective and time-consuming when the number of errors grows up. 

Inspired by the location trajectory coverage metric \cite{covavfuzz}, we also consider the ego car's state (in particular, position and speed) during the simulation rather than the input space variables or human judgement. 
% We report this counting number as the metric to compare the fuzzing methods and give examples to justify this definition.  In particular, we conduct counting based on "spatial-speed trajectory coverage". 
We split the pieces of the lane that ego car drives on into $s$ intervals and the ego car's allowed speed range into $l$ intervals to get a two-dimensional coverage plane with dimensions $\mathbf{1}^{s\times l}$. During the simulation, the ego car's real-time location and speed are recorded at 2Hz. The recorded location-speed data points are then mapped to their corresponding "cells" on the coverage plane. Given all the data points mapped into the cells having the same road interval, their average speed is taken, the corresponding speed-road cell is considered "covered", and the corresponding field on the coverage plane is assigned $1$. Note a simulation's final trajectory representation can have at most $s$ non-zero fields although it has $s\times l$ fields in total.

% \zs{A vector is usually represented by a bold letter or with an arrow on top. There are a lot of regular font "traj"s which are not words or symbols. Use trajectory} 
We denote the trajectory vector associated with the simulation run for a specification $x$ to be $\mathbf{R}(x)$ and define:
\begin{defi}
Two \bugs for the simulations runs on specifications $x_1$ and $x_2$ are considered distinct if $\vert \vert \mathbf{R}(x_1)-\mathbf{R}(x_2)\vert \vert_0 > 0$.
\label{errors_count}
\end{defi}

\begin{figure}[ht]
\centering
    \subfloat[\label{fig:traj_357}]
    {\includegraphics[width=0.034\textwidth]{images/dist/traj_heatmap_357.pdf}}
    \vspace{0.2mm}
    \subfloat[$t_0$]
    {\includegraphics[width=0.14\textwidth]{images/dist/town06_op_357_0/900.jpg}}
    \vspace{0.1mm}
    \subfloat[$t_1$]
    {\includegraphics[width=0.14\textwidth]{images/dist/town06_op_357_0/1000.jpg}}
    \vspace{0.1mm}
    \subfloat[$t_2$]
    {\includegraphics[width=0.14\textwidth]{images/dist/town06_op_357_0/1100.jpg}}

    \subfloat[\label{fig:traj_445}]
    {\includegraphics[width=0.034\textwidth]{images/dist/traj_heatmap_445.pdf}}
    \vspace{0.2mm}
    \subfloat[$t_0$]
    {\includegraphics[width=0.14\textwidth]{images/dist/town06_op_445_30/2100.jpg}}
    \vspace{0.1mm}
    \subfloat[$t_1$]
    {\includegraphics[width=0.14\textwidth]{images/dist/town06_op_445_30/2175.jpg}}
    \vspace{0.1mm}
    \subfloat[$t_2$]
    {\includegraphics[width=0.14\textwidth]{images/dist/town06_op_445_30/2250.jpg}}
\caption{Examples of two \bugs with different trajectories. (a) and (e) show speed-location coverage where the x-axis is speed and y axis is the road interval.}
\label{fig:traj_demo}
\end{figure} 


To demonstrate this error counting approach, we show two \bugs %(found by \tool on \original in \Sa) under the \Cref{fig:motivating_example} scenario 
with different trajectories in \Cref{fig:traj_demo}. 
In both \Cref{fig:motivating_example} and the first row of \Cref{fig:traj_demo}, the ego car hits a bicyclist cutting in from the right lane. The difference is only that the yellow car on the left lane has different behaviors across the two runs. However, the yellow car does not influence the ego car's behavior. Hence, the two simulation runs have the same trajectory coverage (ref. \Cref{fig:traj_357}). 
By contrast, the other \bug on the second row of \Cref{fig:traj_demo} has a different trajectory (ref. \Cref{fig:traj_445}) that the ego car in high speed collides with a motorcycle at a location close to the destination. This example illustrates the necessity of counting \bugs upon \Cref{errors_count}.



% We further manually classify these distinct \bugs based on human judgement as different categories according to root cause and report the number of distinct \bugs categories found by each fuzzing method.





==> body/7_related.tex <==
%!TEX root = main.tex
\section{Related Work}


\subsection{Search}
Search is a classical problem. Numerous methods
When the dimensions become large, 

\subsection{Fuzzing}
Fuzzing generates variations of inputs to search for failure cases for a given software \cite{8449261, Dreossi2019VERIFAIAT}. Fuzzing has been applied to both simple input formats such as audio, image, or video applications \cite{imagefuzz, audiofuzz, videofuzz, fuzzELF} and more complex formats such as cloud service APIs \cite{pythia20}, XML parsers \cite{XMLfuzz} or language compiler \cite{GCCfuzz}, researchers use a grammar-based fuzzing \cite{evgrammarfuzz, 10.1145/1375581.1375607, 10.5555/2362793.2362831, 9154602, 10.1145/1993316.1993532}. Recently, researchers apply the essence of fuzzing on the problem of AV fuzzing. In particular, they develop domain specific fuzzing techniques. In this work, we propose a fuzzing technique targeted to the fusion component of ADAS systems.

 





==> body/back_1_intro.tex <==
\section{Introduction}

% why simulation
% In recent years, \ad companies start to deploy increasingly more self-driving cars on public roads \cite{waymophoenix, baidubeijing}. In order for \ad systems to be safely and comfortably used by the general public on a day-to-day basis, these systems must be made reliable and safe. \ad companies like Waymo have tested their vehicles on road for more than 20 million miles over the years\cite{waymoreport}. However, such large-scale real-world testing can still fail to cover all the corner cases since the testing drives are highly limited to the locations and road conditions. To complement real-world testing, researchers and practitioners have developed many testing methods aiming to find corner cases in a simulation environment \cite{pathgeneration, blackbox19, NEURIPS2018_653c579e, wheelerimportance2019, Abeysirigoonawardena2019Generating, ding2020learning, Kuutti2020, chenbaiming2020, korenadaptive2018, multimodaltest, testing_vision18, interactiontest, nsga2nn}.

% why fusion
% \ez{I feel like 1st and 2nd paragraph has some redundant stuff. I prefer to bring out safety problem  in fusion earlier rather than in the 2nd paragraph. }%for example, Safety is the top priority in AD system. Previous studies on exploring  safety problems of AD systems (cite) have }

% Nowadays, \ad companies start to deploy increasingly more self-driving cars on public roads \cite{waymophoenix, baidubeijing}. 


% the SAE J3016(TM) ”Standard Road Motor Vehicle Driving Automation System Classification and Definition” 

% \cite{saeadlevels}



% Advanced Driver-Assistance Systems (\adas) are human-machine systems that assist drivers in driving and parking functions and have been widely deployed on production passenger vehicles \cite{adas20}. 
% \new{Unlike the full automation promised by Automated Driving Systems (\ads), \adas provides partial automation like adaptive cruise control, lane departure warning, traffic signals recognition, etc.
% They are widely deployed in many modern day vehicles (e.g. 
% Tesla's AutoPilot, Cadillac's Super Cruise, and Comma Two's \op\cite{openpilotconsumerreport}).}
% \adas are developed to increase road safety but they can malfunction and lead to critical consequences. It is thus important to improve the reliability of \adas. In this work, we focus on finding \adas violations caused by its fusion component, which is a less studied area.

Advanced Driver-Assistance Systems (\adas) are human-machine systems that assist drivers in driving and parking functions and have been widely deployed on production passenger vehicles \cite{adas20} (e.g. 
Tesla's AutoPilot, Cadillac's Super Cruise, and Comma Two's \op\cite{openpilotconsumerreport}). 
\new{Unlike the full automation promised by so-called self-driving cars, \adas provides partial automation like adaptive cruise control, lane departure warning, traffic signals recognition, etc., to promote a safe and effortless driving experience. }
Although \adas are developed to increase road safety,  they can malfunction and lead to critical consequences\cite{tesladeaths}. It is thus important to improve the reliability of \adas. 

A typical \adas, as shown in \Cref{fig:fusion_highlevel}, takes inputs from a set of sensors (e.g., camera, radar, etc.) and outputs driving decisions to the controlled vehicle. It usually has a perception module that interprets the sensor data to understand the surroundings, a planning module that plans the vehicle's successive trajectory, and a control module that makes concrete actuator control signals to drive the vehicle. 
Oftentimes individual sensor data could be unreliable under various extreme environments. For example, a camera can fail miserably in a dark environment, in which a radar can function correctly. 
In contrast, a radar can miss some small moving objects due to its low resolution, while a camera usually provides precise measurements in such cases.
To enable an \adas to drive reliably in most environments, researchers have adopted complementary sensors and developed multi-sensor fusion (\msf) methods to aggregate the data from multiple sensors to model the environment more reliably. If a sensor fails, \msf can still work with other sensors to provide reliable information for the downstream modules and enable the \adas to operate safely.

% A typical \adas, as shown in \Cref{fig:fusion_highlevel}, takes inputs from a set of sensors (e.g. camera, radar, etc.), and outputs driving decisions to the controlled vehicle. It usually has a perception module that interprets the sensor data to understand the surroundings, a planning module that plans the vehicle's successive trajectory, and a control module that makes concrete actuator control signals to drive the vehicle. 
% It is believed that individual sensor data could be unreliable under various extreme environments. For example, a camera can fail miserably in a dark environment in which a radar can function properly. A radar usually has low definition and can miss some small moving objects for which a camera can usually provide precise measurements.
% To enable an \adas to drive reliably in most environments, researchers have adopted complementary sensors and developed multi-sensor fusion (\msf) methods to aggregate the data from multiple sensors to model the environment more reliably. If a sensor fails, \msf can still work with other sensors to provide reliable information \edit{for the downstream modules and enable the \adas to operate normally.}


% \zs{can move fusion here and make it concise. For example,"An \ad system, which is depicted in~\Cref{fig:fusion_highlevel}, usually takes in information from a set of sensors (e.g. camera, LiDAR, radar, IMU, GPS, etc.) and outputs control commands to the vehicle. Complementary sensors are used to make sure an AD to drive reliably in most environments even when some of the sensors fail. To reduce the uncertainty of individual sensors, multi-sensor fusion (\msf) is introduced to process the information provided by the rest sensors can still allow the downstream modules and thus the overall system to operate normally."}

% \zs{At the beginning of 2nd paragraph directly point out the fusion problem}


\begin{figure}[ht]
\centering
    {\includegraphics[width=0.49\textwidth]{images/FusionFuzz_Fusion_Highlevel.pdf}}
\caption{The architecture of a typical \adas system.}
\label{fig:fusion_highlevel}
\end{figure} 


% Within the perception module, there is an important component called fusion, which combines processed multiple sensor inputs and models the surrounding environment. 

% Individual sensor input can be unreliable. For example, a camera can fail miserably in a dark environment and a LiDAR can be highly inaccurate on a smoggy day. Complementary sensors are used to make sure an AD to drive reliably in most environments even when some of the sensors fail. To integrate the information from multiple sensors,  multi-sensor fusion (\msf) is introduced to process these information and provides a more reliable modeling of the surrounding to the downstream module and thus allow the overall system to operate normally.


However, \msf hardly knows which sensor provides the most accurate information at each time step. Thus, it neither thoroughly eliminates the uncertainty nor always weighs more on the right sensor data. This inherent flaw may introduce safety risks to the \adas.
In the study of a popular commercial \adas named \op, we found that its default rule-based \msf occasionally produces inaccurate output despite an accurate input exists, and leads the entire system to critical accidents. Similarly, running \op with an alternative Kalman-filter based \msf also suffers from certain fusion-inducing failures. 
To improve the \msf reliability and assure the entire \adas safety in most environments, identifying and understanding such hidden risks are essential, whereas we need to address two primary challenges.


%\zs{To ..., detecting the safety problems of \msf is essential.}

% To improve a \msf reliability and thus the entire \ad system's safety in most environments, detecting such safety problems of \msf is essential.
%\sg{why openpilot and why ADAS?}

\noindent
\textbf{Challenges.} 
% % \ez{It is not straightforward to attribute the causation of a safety violation to fusion module. The input of fusion can be either the raw data such as a sequence of images  captured by a camera, or the synthesized data such as cluttered radar signals. The dynamics of the environment makes the input to fusion module non-deterministic. It is non-trivial to identify a particular environment under which they fail and lead to critical consequences. Also, the output of the fusion module doesn't introduce safety violations directly. It has to pass through other modules like planning, control etc., to determine vehicle's acuation. Thus it is non-trivial to evaluate its impact...}
% {Toward the in-depth reasoning of \msf safety problems in ADAS, we have to tackle several challenges.}\bray{this sentence does not make much sense to me. May be this sentence is redundant as it is already under challenge paragraph.}
% First, it is difficult to pinpoint a safety violation to some imperfect fusions in the \msf component.
% % The input of fusion can be either the raw data such as a sequence of images captured by a camera, or the synthesized data such as cluttered radar signals. 
% The inputs to the fusion component are highly non-deterministic while the output would not directly trigger safety violations since it has to go through planning and control modules to reach the vehicle actuation. 
% %
% Also, the ADAS system dynamics decides that a critical safety violation might happen after the accumulation of many time cycles of system executions. 
% % Thus, it is difficult to evaluate the impact of the fusion component on the entire system's behavior.
% %
% Further, the widely used fusion methods can function properly in many environment conditions. And it is non-trivial to identify the failure cases that cause severe consequences.
% % a particular environment under which they will fail and lead to critical consequences.
% \bray{Can you number the challenges here. It is now all mingled.}
\edit{First, existing fusion methods can function properly most of time so their failure cases are sparse among all the driving situations. Given testing an \ad system is costly, it is non-trivial to identify the failure cases within a limited time budget. Second, it is hard to perform causality forensics between safety violations and the fusion method. The fusion inputs can be highly non-deterministic and the fusion output might not instantly trigger a safety violation because it has to undergo subsequent planning and control modules to take effect. Thus, a critical violation may occur after the accumulation of many cycles of system executions. }






\noindent
\textbf{Our Approach.}
\new{We first address the challenge on the difficulty of finding \bugs, which are defined to be collisions of the \adas caused by its fusion method}. In the driving automation testing domain, recent works leverage fuzz testing (fuzzing) to generate simulator input scenarios to run a target system and search for failure-inducing scenarios \cite{testing_vision18, avfuzzer, covavfuzz, autofuzz21}. 
However, these methods treat the target system as a black-box and ignore the attainable run-time information of the system. Inspired by the grey-box fuzzing in software fuzzing literature \cite{fuzzing_survey}, we propose an evolutionary algorithm-based fuzzing framework \tool \new{(Fusion Error Detector)} that utilizes the input and output information of the fusion component of the system. In particular, we propose a novel objective function that simultaneously maximizes the deviation of the fusion output from the ground-truth, and minimizes the deviation of a fusion input from the ground-truth. Intuitively, when both objectives are met, the fusion method must have made a bad decision since it fails to utilize the more accurate input to generate an accurate output. If the simulation then witnesses an error of the auto-driving car, the fusion output is the likely cause. 
% Consequently, \tool can greatly ease the efforts in detecting \bugs. 


% %To determine if an error truly stems from the misbehavior of the fusion method, 
% Inspired by the counterfactual theories of causation, we compare the entire \adas behavior between the original fusion method and an oracle-like fusion method in an otherwise identical setting, respectively. The behavioral differences would stem from the fusion methods. We call an error under such context a \emph{\bug}.
% %
% To perform a reproducible comparison, we leverage the high-fidelity simulator \carla~\cite{carla} to construct a stable virtual safety testing~\cite{covavfuzz} environment.
% ~\bray{This para will be very confusing to a reader who does not know causality. Can you give a bit more intuition?}
% %Similar problem has been encountered in finding bugs of software.
% To approach the stateful failure cases by applying tactic simulator traffic to the \adas executions, we adopt the fuzz testing (fuzzing) approach.
% %
% Fuzzing generates input variations and searches for execution failures with application dependent objective functions \cite{8449261, Dreossi2019VERIFAIAT}. Recent works developed auto-driving scenario fuzzing and identified incidents using evolutionary algorithms with domain-specific objectives \cite{testing_vision18, avfuzzer}.
% %
% In this work, we extend the general idea of auto-driving specification fuzzing and propose an evolutionary-based fuzzing algorithm to detect safety problems that span many execution cycles~\bray{very unclear....all I get is some buzz words}.
% Moreover, we leverage the attainable information of the fusion component in an \adas system to enhance our fuzzing technique. Previous fuzzing methods often treat the auto-driving system as a black-box and ignore the helpful information from the system \cite{testing_vision18, avfuzzer}. Inspired by the grey-box fuzzing that utilizes system statistics in software fuzzing literature \cite{fuzzing_survey}, we propose a new fuzzing method \tool that drastically eases the detecting effort of \bugs. 
% \bray{It is not clear at all how fuzzing and causality is related.}
% \zs{We adapt counterfactual theories of causation [citation] to solve the first challenge. That is, we study if an error will still happen if the }
To address the challenge of error attribution, we study if an error still happens after we replace the original fusion method with a proposed fusion method in an otherwise identical setting in a simulation environment. 
% In the counterfactual theories of causation, an event A causes an event B, if and only if, if A were not to occur B would not occur. 
\new{Based on the theory of causality analysis, we construct a causal graph involving all the variables potentially influencing the occurrence of a collision during a simulation. We next show that after the replacement, given everything else stays the same, if the error no longer happens in the simulation, the original fusion method would be considered the cause of the original error.  
To ensure elements other than the fusion method can be controlled to be identical between the original run and a new run, we apply an intervention via setting the communications between the studied \adas, \op, and the used high-fidelity simulator \carla~\cite{carla} to be deterministic and synchronous for all the simulations. To efficiently find a fusion method that can avoid the collision, we propose to use a \emph{best-sensor fusion} method which always selects the sensor's output that is closest to the ground-truth.}



% Fuzzing generates input variations and searches for execution failures with application dependent objectives \cite{8449261, Dreossi2019VERIFAIAT}. Recent works developed auto-driving scenario fuzzing and identified accidents using evolutionary algorithms with domain-specific objectives \cite{avfuzzer, covavfuzz}. In this work, we extend the general idea of auto-driving scenario fuzzing and propose an evolutionary-based fuzzing algorithm to detect \bugs.


%use search objectives like minimum obstacle distance \cite{avfuzzer, testing_vision18} to find collisions. These methods, however, 

To the best of our knowledge, our technique is the first fuzzing method targeting the \adas fusion component.
% Based on the insights we have gain from \bugs found on the studied fusion methods, we further make a small changes to it and the improved fusion method successfully avoids many of found \bugs.
% Previous work on simulation testing \cite{pathgeneration, blackbox19, NEURIPS2018_653c579e, wheelerimportance2019, Abeysirigoonawardena2019Generating, ding2020learning, Kuutti2020, chenbaiming2020, korenadaptive2018, multimodaltest, testing_vision18, interactiontest, nsga2nn} constructs a parametrized space which usually consists of the environment variables like the weather and actor behavior variables like their initial locations and velocity. We extend the NPC vehicles changing lane scenarios from \cite{avfuzzer} since those usually provide complex actor's interaction.
In summary, we make the following contributions:
\begin{itemize}
\item \new{We define \emph{\bugs} and develop \tool, a novel grey-box testing framework for efficiently revealing \emph{\bugs} in \adas}
\item \new{We analyze the definition of \emph{\bugs} using causality analysis and justify it.}
\item \new{We evaluate \tool on two popular fusion methods in an industry-grade \adas, and show that it can disclose safety issues and find more \bugs than baselines.}
\item We propose suggestions to mitigate \emph{\bugs} and effectively reduce  \emph{\bugs} in a preliminary study.
\end{itemize}

The source code of our tool and interesting findings are available at \url{https://github.com/FusionFuzz/FusionFuzz}.
